Partially Observable Markov Decision Process Modelling for Assessing Hierarchies

Hierarchical clustering has been shown to be valuable in many scenarios. Despite its usefulness to many situations, there is no agreed methodology on how to properly evaluate the hierarchies produced from different techniques, particularly in the case where ground-truth labels are unavailable. This motivates us to propose a framework for assessing the quality of hierarchical clustering allocations which covers the case of no ground-truth information. This measurement is useful, e.g., to assess the hierarchical structures used by online retailer websites to display their product catalogues. Our framework is one of the few attempts for the hierarchy evaluation from a decision-theoretic perspective. We model the process as a bot searching stochastically for items in the hierarchy and establish a measure representing the degree to which the hierarchy supports this search. We employ Partially Observable Markov Decision Processes (POMDP) to model the uncertainty, the decision making, and the cognitive return for searchers in such a scenario.

==> amazon_1_hqs_table.tex <==
\begin{table}[h]
\centering
\caption{Summary of HQS for Hierarchy A} \label{tb:amazon-1-hqs}
\begin{tabular}{lrr}
\toprule
$x$ &  Stop at &   $V(x)$ \\
\midrule
0  &        3 &  0.620389 \\
1  &        4 &  0.746515 \\
2  &        4 &  0.826451 \\
3  &        4 &  0.811422 \\
4  &        3 &  0.599822 \\
5  &        4 &  0.517870 \\
6  &        4 &  0.792900 \\
7  &        2 & -0.679057 \\
8  &        2 &  0.561567 \\
9  &        3 &  0.431666 \\
10 &        4 &  0.812053 \\
11 &        4 &  0.816681 \\
\bottomrule
\end{tabular}
\end{table}


==> amazon_2_hqs_table.tex <==
\begin{table}[h]
\centering
\caption{Summary of HQS for Hierarchy B} \label{tb:amazon-2-hqs}
\begin{tabular}{lrr}
\toprule
$x$ &  Stop at &   $V(x)$ \\
\midrule
0  &        1 &  0.000000 \\
1  &        3 & -0.991150 \\
2  &        3 & -0.988855 \\
3  &        2 & -0.862852 \\
4  &        3 & -0.955350 \\
5  &        3 & -0.736097 \\
6  &        3 &  0.759935 \\
7  &        3 &  0.658529 \\
8  &        2 & -0.995267 \\
9  &        1 &  0.000000 \\
10 &        3 &  0.749206 \\
11 &        1 &  0.000000 \\
\bottomrule
\end{tabular}
\end{table}


==> amazon_3_hqs_table.tex <==

\begin{table}[h]
\centering
\caption{Summary of HQS for Hierarchy C} \label{tb:amazon-3-hqs}
\begin{tabular}{lrr}
\toprule
$x$ &  Stop at &   $V(x)$ \\
\midrule
0  &        2 & -0.751922 \\
1  &        2 & -0.999094 \\
2  &        1 &  0.000000 \\
3  &        1 &  0.000000 \\
4  &        1 &  0.000000 \\
5  &        2 &  0.889234 \\
6  &        2 & -0.856630 \\
7  &        2 & -0.933072 \\
8  &        2 &  0.878909 \\
9  &        1 &  0.000000 \\
10 &        2 & -0.964455 \\
11 &        2 & -0.978953 \\
\bottomrule
\end{tabular}
\end{table}


==> amazon_4_hqs_table.tex <==
\begin{table}[h]
\centering
\caption{Summary of HQS for Hierarchy D} \label{tb:amazon-4-hqs}
\begin{tabular}{lrr}
\toprule
$x$ &  Stop at &   $V(x)$ \\
\midrule
0  &        3 & -0.668088 \\
1  &        2 & -0.740265 \\
2  &        3 & -0.707562 \\
3  &        3 & -0.995524 \\
4  &        3 & -0.651974 \\
5  &        3 & -0.999896 \\
6  &        2 & -0.791041 \\
7  &        2 & -0.807062 \\
8  &        2 & -0.995364 \\
9  &        2 & -0.925345 \\
10 &        2 & -0.989777 \\
11 &        3 & -0.900619 \\
\bottomrule
\end{tabular}
\end{table}


==> amazon_5_hqs_table.tex <==
\begin{table}[ht]
\centering
\caption{Summary of HQS for Hierarchy E} \label{tb:amazon-5-hqs}
\begin{tabular}{lrr}
\toprule
{} &  Stop at &      V(x) \\
\midrule
0  &        3 &  0.610799 \\
1  &        3 & -0.797205 \\
2  &        4 &  0.672706 \\
3  &        1 &  0.000000 \\
4  &        3 &  0.533369 \\
5  &        1 &  0.000000 \\
6  &        2 &  0.833914 \\
7  &        1 &  0.000000 \\
8  &        2 &  0.423173 \\
9  &        1 &  0.000000 \\
10 &        2 &  0.834673 \\
11 &        4 &  0.807958 \\
\bottomrule
\end{tabular}
\end{table}


==> amzon_table.tex <==
\begin{table}[!ht]
\centering
\caption{Selected Items from Amazon: Part 1}\label{tb:amazon1}
\small
\input{amazon_table_1}
\end{table}

\begin{table}[!ht]
\centering
\caption{Selected Items from Amazon: Part 2}\label{tb:amazon2}
\small
\input{amazon_table_2}
\end{table}


==> design.tex <==
% !TEX root =  evalmodel.tex
\section{HQS Design Summary}
\label{sec:design}
To summarise the motivation and methodology behind  our proposed HQS measure,~\cref{tb:design} lists the challenges we have addressed and how these have been handled within our proposed framework.

\begin{table}[!ht]
\centering
\caption{Design of HQS}\label{tb:design}
\small
% \begin{tabularx}{1.1\textwidth}{X X X X}
\begin{tabular}{p{1.6cm} p{2.cm} p{3.5cm} p{3.3cm}}
\textsc{Aspect} & \textsc{Requirement} & \textsc{Challenge} & \textsc{Solution} \\
\toprule
Practical implementation & Tractability & Solving a POMDP is universally intractable & Online planner to guarantee sub-optimality \\
\midrule
Practical implementation & Flexibility in the guidance function & Different traditional measures may fit specific datasets better than others & Leave the similarity choice to the users \\
\midrule
Practical implementation & Fair probabilities from the feedback & It could happen that cluster qualities are equally bad as the bot descends. For example, the similarities of $x$ to random cluster A and cluster B, respectively, return $10^{-50}$ and $10^{-70}$, but then A will have the probability $\eta = 1$ & Use Boltzmann distribution and tune the temperature parameter to control this situation---temperature can be also a function over time (current depth of the hierarchy) $t$, e.g. $\delta_t \triangleq \delta_{base}\nu^{t}$ where $\nu \in [1, \infty)$ \\
\midrule
Measuring need & Uncertainty in the bot's search & Stochastic policies are hardly studied; There is no way to judge it & Impose the randomness into the bot's moving actions \\
\midrule
Measuring need & Limit the bot not to be too smart & E.g., POMCP ignores the external belief and guides the bot to find the target with a high probability & Greedy optimisation---RTBSS \\
\bottomrule
\end{tabular}
\end{table}


==> rewarddesign.tex <==
\paragraph{Reward Function}

Consider a scenario in which $q(c, c') = \gamma$, a constant at each step of the hierarchical search.  Hence, at level $\ell$ (i.e. after $\ell$ steps of the search, starting at $\ell=0$), the probability of being on the right path is $\gamma^\ell$.  Using $r_\ell$ to represent the reward obtained for successfully finding the target at this step, the value function for a strategy that stops at this step can be written as:
\begin{align*}
  V = \gamma^\ell r_\ell + ( 1 - \gamma^\ell) (-1) = \gamma^\ell(r_\ell +1) - 1
\end{align*}
 since with probability $1 - \gamma^\ell$, the searcher is on a wrong path and obtains reward of $-1$.

 Further we'll assume that the reward grows geometrically as the target is found at deeper levels.
 %This might be the case when documents are distributed so that the number of documents stored under a node at the $\ell^{\rm th}$ level is $\alpha^\ell D$ where $D$ is the full dataset size.
 The reward is given as
 \begin{align*}
   r_\ell = \beta(1 - \alpha)
 \end{align*}
where $\alpha$ is the searching effort score and $\beta$ is a scale coefficient in accordance to the adventure sensation.
Also, we retain $0\le \alpha \le 1$ and  $0 \le \beta \le 1$.
However, we would like $\beta$ to be dependent on $\ell$.
Besides, we would not like to penalize stopping too early, we retain a golden ratio number as a bottom line such that
\begin{align}
  \beta = (6.18 + \gamma^{-g\ell})
\end{align}
where $0 \le \gamma^{-g\ell} \le 0.382$.

We can now write the value function as
\begin{align*}
  V &= \gamma^\ell((6.18 + \gamma^{-g\ell})(1 - \alpha) + 1) - 1 \\
    &= (0.618\gamma^\ell + \gamma^{\ell(1-g)})(1 - \alpha) + \gamma^\ell - 1  \,.
\end{align*}

\begin{align*}
  \frac {dV} {d\ell} &= (1-\alpha) [0.618\ln(\gamma) \gamma^\ell + (1-g)\ln(\gamma) (\gamma)^{\ell(1-g)}] + \ln(\gamma) \gamma^\ell\\
  \frac {dV} {d\ell} &= 0 \implies \\
   0  &= \ln(\gamma) \gamma^\ell \{(1 - \alpha) [0.618  + (1-g)\gamma^{-g\ell}] + 1\} \\
   \gamma^{-g\ell} &=  \frac {\frac 1 {\alpha - 1} - 0.618} {1-g} \\
   &= \frac {1.618 - 0.618 \alpha} {(1 - g)(\alpha - 1)} \\
   \ell_{\rm opt} &= - \frac {\ln \frac {1.618 - 0.618 \alpha} {(1 - g)(\alpha - 1)}} {g\ln \gamma} \\
   &= \frac {\ln[(1 - g)(\alpha - 1)]}  {g\ln \gamma} - \frac {\ln(1.618 - 0.618 \alpha)}  {g\ln \gamma}
\end{align*}
If $V$ is monotonically decreasing, there is no motivation to search the hierarchy. Similarly, if it is monotonically increasing, then the searcher will be motivated to explore the entire hierarchy to the leaf nodes. On the other hand, there may be some level $\ell$ at which $V$ is maximised. The situation depends on the relationship between $\alpha$ and $\gamma$.  To make this relationship explicit, write
\[
	\alpha = \gamma^g
\]
for some $g \in [0,\infty)$.  Differentiating with respect to $\ell$, we find a turning point at $\ell_{\rm opt}(g)$ when
\begin{align*}
                0 &= (2 - \gamma^{g\ell}) \gamma^\ell \log \gamma + \gamma^\ell (-g\gamma^{g \ell} \log\gamma)  \\
                0 &= 2  - (1 + g) \gamma^{g\ell} \\
                \ell_{\rm opt}(g) &= \frac 1 {g\log \gamma} \left(\log 2 - \log (1+g)\right)
\end{align*}
For a turning point in the range $\ell\ge 0$, we therefore require that $g\ge 1$.  Note that as $\gamma \to 1$, i.e. we are more certain to take the correct path, $\ell_{\rm opt} \to \infty$.

In the interest of exploring as much of the tree as possible, we can also ask what value of $g$ maximises $\ell_{\rm opt}$.  Differentiating $\ell_{\rm opt}(g)$ with respect to $g$, we obtain a maximum when
\begin{align*}
             0 &= g + (1+g)(\log 2 - \log (1+g) )
\end{align*}
which occurs for  $g^*$ between 3 and 4.  For this optimal value of $g$, we have that
\begin{align*}
             0 &= g^* + (1+g^*)(g^* \ell_{\rm opt}(g^*) \log\gamma  )\\
             \ell_{\rm opt}(g^*) &= \frac 1 {(1+g^*)(-\log \gamma)}
 \end{align*}

 Note that in this model, we have
 \begin{align}
 \label{eqn:rewardfunc}
     r_{\ell} = 1 - \gamma^{g\ell} = 1 - \mathrm{Prob}(\mbox{correct path at step } \ell)^g
 \end{align}
 for $g\ge 1$. This shows that, in order for there to be a turning point in the value function, the reward should increase more rapidly than the probability of being on the right path decreases. It makes sense that the reward should compensate the risk of descending the levels, when finally we stop on a correct path. This simple analysis supports that a reward of the form of (\ref{eqn:rewardfunc}) should be adopted.  In this case, the parameter $g$ could be chosen as a function of the number of documents at the node, with fewer documents implying a larger $g$.


 \paragraph{Reward Function}

 Consider a scenario in which $q(c, c') = \gamma$, a constant at each step of the hierarchical search.  Hence, at level $\ell$ (i.e. after $\ell$ steps of the search, starting at $\ell=0$), the probability of being on the right path is $\gamma^\ell$.  Using $r_\ell$ to represent the reward obtained for successfully finding the target at this step, the value function for a strategy that stops at this step can be written as:
 \begin{align*}
           V = \gamma^\ell r_\ell + ( 1 - \gamma^\ell) (-1) = \gamma^\ell(r_\ell +1) - 1
 \end{align*}
  since with probability $1 - \gamma^\ell$, the searcher is on a wrong path and obtains reward of $-1$.

  Further we'll assume that the reward grows geometrically as the target is found at deeper levels.
  %This might be the case when documents are distributed so that the number of documents stored under a node at the $\ell^{\rm th}$ level is $\alpha^\ell D$ where $D$ is the full dataset size.
  The reward is given as
  \begin{align*}
         r_\ell = 1 - \alpha^\ell
  \end{align*}
  for some $0\le \alpha \le 1$. We can now write the value function as
  \begin{align*}
           V = \gamma^\ell(2 - \alpha^\ell) - 1\,.
 \end{align*}
 If $V$ is monotonically decreasing, there is no motivation to search the hierarchy. Similarly, if it is monotonically increasing, then the searcher will be motivated to explore the entire hierarchy to the leaf nodes. On the other hand, there may be some level $\ell$ at which $V$ is maximised. The situation depends on the relationship between $\alpha$ and $\gamma$.  To make this relationship explicit, write
 \[
 	\alpha = \gamma^g
 \]
 for some $g \in [0,\infty)$.  Differentiating with respect to $\ell$, we find a turning point at $\ell_{\rm opt}(g)$ when
 \begin{align*}
                 0 &= (2 - \gamma^{g\ell}) \gamma^\ell \log \gamma + \gamma^\ell (-g\gamma^{g \ell} \log\gamma)  \\
                 0 &= 2  - (1 + g) \gamma^{g\ell} \\
                 \ell_{\rm opt}(g) &= \frac 1 {g\log \gamma} \left(\log 2 - \log (1+g)\right)
 \end{align*}
 For a turning point in the range $\ell\ge 0$, we therefore require that $g\ge 1$.  Note that as $\gamma \to 1$, i.e. we are more certain to take the correct path, $\ell_{\rm opt} \to \infty$.

 In the interest of exploring as much of the tree as possible, we can also ask what value of $g$ maximises $\ell_{\rm opt}$.  Differentiating $\ell_{\rm opt}(g)$ with respect to $g$, we obtain a maximum when
 \begin{align*}
              0 &= g + (1+g)(\log 2 - \log (1+g) )
 \end{align*}
 which occurs for  $g^*$ between 3 and 4.  For this optimal value of $g$, we have that
 \begin{align*}
              0 &= g^* + (1+g^*)(g^* \ell_{\rm opt}(g^*) \log\gamma  )\\
              \ell_{\rm opt}(g^*) &= \frac 1 {(1+g^*)(-\log \gamma)}
  \end{align*}

  Note that in this model, we have
  \begin{align}
  \label{eqn:rewardfunc}
      r_{\ell} = 1 - \gamma^{g\ell} = 1 - \mathrm{Prob}(\mbox{correct path at step } \ell)^g
  \end{align}

